JobComposer: Career Path Optimization via Multicriteria Utility Learning

With online professional network platforms (OPNs, e.g., LinkedIn, Xing, etc.) becoming popular on the web, people are now turning to these platforms to create and share their professional profiles, to connect with others who share similar professional aspirations and to explore new career opportunities. These platforms however do not offer a long-term roadmap to guide career progression and improve workforce employability. The career trajectories of OPN users can serve as a reference but they are not always optimal. A career plan can also be devised through consultation with career coaches, whose knowledge may however be limited to a few industries. To address the above limitations, we present a novel data-driven approach dubbed JobComposer to automate career path planning and optimization. Its key premise is that the observed career trajectories in OPNs may not necessarily be optimal, and can be improved by learning to maximize the sum of payoffs attainable by following a career path. At its heart, JobComposer features a decomposition-based multicriteria utility learning procedure to achieve the best tradeoff among different payoff criteria in career path planning. Extensive studies using a city state-based OPN dataset demonstrate that JobComposer returns career paths better than other baseline methods and the actual career paths.

==> figures/benchmark_table.tex <==
\begin{tabular}{llrrlrrlrrl}
\toprule
{} &                                             Method &  D\_avg &  D\_median & D\_p-value &  L\_avg &  L\_median & L\_p-value &  R\_avg &  R\_median & R\_p-value \\
\midrule
0 &                                 Greedy most common & -88.80 &    -48.00 &  0.00e+00 &  11.67 &      0.00 &  1.32e-40 &  -0.07 &      0.00 &  0.00e+00 \\
1 &                           Greedy shortest duration &  23.06 &     24.00 &  0.00e+00 &   2.67 &      0.00 &  0.00e+00 &  -0.32 &     -0.19 &  0.00e+00 \\
2 &                                  Greedy level gain & -28.39 &     -2.00 &  0.00e+00 &  26.84 &      4.85 &  0.00e+00 &  -0.34 &     -0.20 &  0.00e+00 \\
3 &                           Greedy desirability gain & -57.38 &    -59.51 &  0.00e+00 &  19.19 &      5.16 &  0.00e+00 &   0.96 &      1.05 &  0.00e+00 \\
4 &              Single-criterion utility (\$-D\_\{s,d\}\$) &  61.30 &     49.00 &  0.00e+00 &  -6.55 &      0.00 &  0.00e+00 &  -0.49 &     -0.35 &  0.00e+00 \\
5 &               Single-criterion utility (\$L\_\{s,d\}\$) & -90.45 &    -43.00 &  0.00e+00 &  81.52 &     20.50 &  0.00e+00 &  -0.34 &     -0.19 &  0.00e+00 \\
6 &               Single-criterion utility (\$R\_\{s,d\}\$) & -36.65 &    -38.33 &  0.00e+00 &   5.96 &      0.00 &  0.00e+00 &   1.10 &      1.23 &  0.00e+00 \\
7 &  Equally weighted utility (\$L\_\{s,d\} - D\_\{s,d\} +... & -42.83 &    -51.50 &  0.00e+00 &  12.31 &      0.30 &  0.00e+00 &   1.09 &      1.22 &  0.00e+00 \\
8 &  Multicriteria utility (\$[-D\_\{s,d\}, L\_\{s,d\}, R\_... & -26.43 &    -33.07 &  0.00e+00 &  10.48 &      0.00 &       - &   1.10 &      1.23 &  0.00e+00 \\
\bottomrule
\end{tabular}


==> figures/benchmark_table_ws_sum.tex <==
\begin{tabular}{llrrlrrlrrlr}
\toprule
{} &                                             Method &  D\_avg &  D\_median & D\_p-value &  L\_avg &  L\_median & L\_p-value &  R\_avg &  R\_median & R\_p-value &          PIM \\
\midrule
0 &                                 Greedy most common & -88.80 &    -48.00 &  0.00e+00 &  11.67 &      0.00 &  0.00e+00 &  -0.07 &      0.00 &  0.00e+00 &    74.010889 \\
1 &                           Greedy shortest duration &  23.06 &     24.00 &  0.00e+00 &   2.67 &      0.00 &  0.00e+00 &  -0.32 &     -0.19 &  0.00e+00 &   -19.458482 \\
2 &                                  Greedy level gain & -28.39 &     -2.00 &  0.00e+00 &  26.84 &      4.85 &  0.00e+00 &  -0.34 &     -0.20 &  0.00e+00 &   255.369754 \\
3 &                           Greedy desirability gain & -57.38 &    -59.51 &  0.00e+00 &  19.19 &      5.16 &  3.34e-04 &   0.96 &      1.05 &  0.00e+00 & -1057.248676 \\
4 &              Single-criterion utility (\$-D\_\{s,d\}\$) &  61.30 &     49.00 &  0.00e+00 &  -6.55 &      0.00 &  0.00e+00 &  -0.49 &     -0.35 &  0.00e+00 &   198.449126 \\
5 &               Single-criterion utility (\$L\_\{s,d\}\$) & -90.45 &    -43.00 &  0.00e+00 &  81.52 &     20.50 &  0.00e+00 &  -0.34 &     -0.19 &  0.00e+00 &  2478.660890 \\
6 &               Single-criterion utility (\$R\_\{s,d\}\$) & -36.65 &    -38.33 &  0.00e+00 &   5.96 &      0.00 &  0.00e+00 &   1.10 &      1.23 &  0.00e+00 &  -240.306304 \\
7 &  Equally weighted utility (\$L\_\{s,d\} - D\_\{s,d\} +... & -42.83 &    -51.50 &  0.00e+00 &  12.31 &      0.30 &  0.00e+00 &   1.09 &      1.22 &  0.00e+00 &  -577.012735 \\
8 &  Multicriteria utility (\$[-D\_\{s,d\}, L\_\{s,d\}, R\_... &  16.36 &      7.00 &       nan &  19.51 &      1.00 &       nan &   0.76 &      0.81 &       nan &   241.727230 \\
\bottomrule
\end{tabular}

